Adaptive Invariance for Molecule Property Prediction

Effective property prediction methods can help accelerate the search for COVID-19 antivirals either through accurate in-silico screens or by effectively guiding on-going at-scale experimental efforts. However, existing prediction tools have limited ability to accommodate scarce or fragmented training data currently available. In this paper, we introduce a novel approach to learn predictors that can generalize or extrapolate beyond the heterogeneous data. Our method builds on and extends recently proposed invariant risk minimization, adaptively forcing the predictor to avoid nuisance variation. We achieve this by continually exercising and manipulating latent representations of molecules to highlight undesirable variation to the predictor. To test the method we use a combination of three data sources: SARS-CoV-2 antiviral screening data, molecular fragments that bind to SARS-CoV-2 main protease and large screening data for SARS-CoV-1. Our predictor outperforms state-of-the-art transfer learning methods by significant margin. We also report the top 20 predictions of our model on Broad drug repurposing hub.

==> backup.tex <==
\section{Domain Extrapolation}
In many applications, training data is often limited and biased due to experimental constraints. Therefore, it is important to ensure that the model predictions generalize substantially beyond training data. For instance, in computational chemistry, property prediction models are often evaluated under scaffold split~\cite{bemis1996properties}: models are evaluated on compounds with new scaffolds unseen during training in order to measure model's extrapolation capability. In this case, scaffold divides the chemical space into multiple domains and the model needs to learn to extrapolate beyond the domains in the training set. This is very challenging because scaffold is a combinatorial object and the number of domains often scales linearly to the training set size.

The key to achieve domain extrapolation is to enforce the right invariance constraint during training. So far the community has explored roughly three strategies to facilitate extrapolation: 
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=0pt]
    \item Domain adversarial training~\cite{ganin2016domain} enforces the latent representation $Z = \phi(X)$ to have the same distribution across different domains $E$ (i.e., $Z \perp E$). Since all the domains shares the same predictor, the label distribution $P(Y)$ will also be the same across different domains. This is problematic when the training and test domain has very different label distributions~\cite{zhao2019learning}. 
    \item Conditional domain adaptation~\cite{long2018conditional} fixes the above issue by enforcing invariance conditioned on class labels: $Z \perp E \;|\; Y$. This allows the label distribution to vary between different domains. However, this requires the latent representation $Z$ to encode zero information about $E$. This is an unreasonably strong constraint in molecule property prediction where domains are indexed by scaffolds. In fact, the encoder must map different scaffold graphs into the same vector $Z$. 
    \item Invariant risk minimization (IRM)~\cite{arjovsky2019invariant} seeks a different notion of invariance. IRM requires the predictor $f$ to be simultaeously optimal across different domains (environments). Essentially, IRM enforces a conditional independence $Y \perp E \;\vert\; Z$. This allows the latent representation $Z$ to preserve some scaffold information and the label distribution to vary across different scaffolds.
\end{itemize}

While IRM provides a suitable invariance for domain extrapolation, direct application of IRM still has two limitations. First, it assumes each environment has sufficient number of training examples. This does not hold in practice when domains are indexed by combinatorial structures like molecular scaffolds. Due to the sparsity of scaffold distribution, many environments will have only one molecule. Second, due to latent confounding, conditioning on environment $E$ may also change other variables. For example, when conditioning on scaffolds, the molecular weight changes accordingly. As a result, when splitting dataset into different environments, IRM will enforce invariance against other undesired variables as well. In order for IRM to succeed, it is important to curate environments in a controlled manner to avoid the aforementioned issues.



\section{Contrastive IRM}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/IRM.png}
    \caption{\textbf{Left}: Illustration of base GCN model for property prediction. \textbf{Right}: Contrastive IRM. The model perturbs the representation $\phi(x)$ into $\psi(x)$ using the gradient from scaffold classifier $p(s | x)$. The predictor $f$ is trained to be simultaneously optimal across two environments.}
    \label{fig:irm}
\end{figure}

Based on these observations, we propose contrastive IRM that estimates a predictor that is simultaneous optimal (invariant) across different environments.
To address the latent confounding issue, it is important to curate environments in a controlled manner similar to an intervention.
Specifically, we require the predictor to be optimal across two environments: the original training set $\{(x_i,y_i)\}$ and a perturbed version of this set. 
Conceptually, the perturbed training set can be viewed as applying scaffold intervention to input molecules. %consists of virtual compounds with the same labels but with modified scaffolds. 
As molecular graphs are discrete and thus challenging to operate on directly, we instead introduce perturbations in their associated continuous representations $\phi$. The manner of perturbation is specifically tailored to facilitate generalization across scaffolds. Indeed, we modify the vector representation of each compound so as to make its inferred scaffold less distinct according to an auxiliary scaffold classifier $g$: 
\begin{equation}
    \psi(x) = \phi(x) - \alpha \nabla_{\phi(x)} g(\phi(x))
\end{equation}
The scaffold classifier $g$ is trained to predict the correct scaffold for each molecule $x$ based on the molecule's vector representation $\phi(x)$. The perturbed representation of $x$, i.e., $\psi(x)$ corresponds to a more generic (virtual) scaffold by construction, yet it ought to be classified the same. Both the original and virtual representations are fed to a feed-forward network $f$ for final activity prediction. 

We begin by introducing invariant prediction and then incorporate scaffold perturbation explicitly into this framework. To this end, we define the classification losses associated with the original and perturbed molecules ($\ell$ can be any loss function):
\begin{equation}
    \mathcal{L}(f\circ h) = \sum_{(x,y)\in \mathcal{D}} \ell(y, f(h(x))) \qquad h\in \{\phi, \psi\}
\end{equation}
Similar to \cite{arjovsky2019invariant}, our contrastive IRM method seeks to find a representation $\phi(\cdot)$ and the associated feed-forward predictor $f$ such that $f$ would be simultaneously optimal across the two ``environments'' (original and perturbed):
\begin{equation}
    \min_{\phi,f} \sum_{h \in \{\phi,\psi\}}\mathcal{L}(f \circ h) \qquad \mathrm{s.t.}\;\; \forall h: f \in \arg\min_{f_h} \mathcal{L} (f_h \circ h)
\end{equation}
where $\psi$ (perturbed representation) is always a function of the original $\phi$. Since the optimality condition is equivalent to $\mathcal{L}(f \circ h) \leq \min_{f_h} \mathcal{L}(f_h \circ h)$, we can turn this bi-level optimization problem into an easier to solve version through the use of Lagrange multipliers: 
\begin{equation}
    \min_{\phi,f} \max_{f_\phi,f_\psi} \sum_{h \in \{\phi, \psi\}} (1 + \lambda_h) \mathcal{L}(f \circ h) - \lambda_h \mathcal{L}(f_h \circ h)
\end{equation}
where $f_\phi$ and $f_\psi$ are environment specific competing predictors that ought not to succeed any better than $f$ if indeed $f$ remains optimal in each environment. Finally, we incorporate the scaffold classifier $g$ into the overall objective. Note that the perturbed representations $\psi(x)$ corresponding to virtual scaffolds depend on both $\phi(x)$ and the scaffold classifier $g$, as defined above.
\begin{equation}
    \min_{\phi,f,g} \max_{f_\phi,f_\psi} \;\; \lambda_s \mathcal{L}^s(g \circ \phi) + \sum_{h \in \{\phi, \psi\}} (1 + \lambda_h) \mathcal{L}(f \circ h) - \lambda_h \mathcal{L}(f_h \circ h)
    \label{eq:cirm}
\end{equation}
Here $\mathcal{L}^s(g \circ \phi)$ is the scaffold classification error on the molecules in the training set. 
Since scaffold is a combinatorial object and the vocabulary of scaffolds is large, we train the scaffold classifier via contrastive learning~\cite{oord2018representation}. Specifically, for a given molecule $x_i$ with scaffold $s_i$, we randomly sample $n$  other molecules and take their scaffolds  $\{s_k\}$ as negative examples. The classifier $g$ consists of a two layer MLP $g_s(\cdot)$ which outputs
\begin{equation}
    g(\phi(x_i)) = \log \frac{\exp(\mathrm{sim}(g_s(\vz_{x_i}), g_s(\vz_{s_i}))}{\sum_{k\neq i} \exp(\mathrm{sim}(g_s(\vz_{x_i}), g_s(\vz_{s_k}))} \qquad \vz_{x_i} = \phi(x_i),\vz_{s_k} = \phi(s_k)
\end{equation}
where $\mathrm{sim(\cdot,\cdot)}$ stands for cosine similarity. In practice, we use the molecules within the same batch as negative examples. 
The above minimax game can be solved through alternating gradient updates between $\phi,f,g$ and competing classifiers $f_\phi,f_\psi$. The training procedure is shown in Algorithm 1.

\begin{algorithm}[t]
\label{alg:cirm}
\begin{algorithmic}[1]
\caption{Contrastive IRM training}
\FOR{each training step}
\STATE Sample a batch of molecules $\{x_1,\cdots,x_n\}$ with their scaffolds $\{s_1,\cdots,s_n\}$
\STATE Encode molecules $\{x_1,\cdots,x_n\}$ into vectors $\{\phi(x_1),\cdots,\phi(x_n)\}$
\STATE Computed scaffold classification loss $\mathcal{L}^s(g \circ \phi) = -\sum_i g(\phi(x_i))$.
\STATE Construct perturbed representation $\psi(x_i) = \phi(x_i) - \alpha \nabla_{\phi(x_i)} g(\phi(x_i))$
\STATE Compute invariant predictor loss $\mathcal{L}(f \circ \phi)$
\STATE Compute competing predictor loss $\mathcal{L}(f_\phi \circ \phi), \mathcal{L}(f_\psi \circ \psi)$
\STATE Update $\phi, f, g$ to minimize Eq.~(\ref{eq:cirm})
\STATE Update $f_\phi, f_\psi$ to maximize Eq.~(\ref{eq:cirm})
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Application to molecule property prediction}
Now we describe how to apply our method to the property prediction task. The training data is a collection of pairs $\{(x_i,y_i)\}$, where $x_i$ is a compound and $y_i$ is its activity score, typically binary (active/inactive).
The feature extractor $\phi(\cdot)$ is a graph convolutional network (GCN) which translates a molecular graph into a continuous vector through directed message passing operations~\cite{yang2019analyzing}. The predictor $f$ is a feed-forward network $f$ that takes $\phi(x)$ as input and predict the activity $y$. 

Specifically, GCN iteratively updates atom and bond representations through messages that aggregate information (features) of neighboring atoms and bonds. 
By applying the message passing operations multiple times, the model effectively collects together information from broader neighborhoods around each atom. The highest-level messages are then combined into a single continuous vector $\phi(x)$ that represents the entire molecule $x$ (Figure~\ref{fig:irm}). 
